Improving Maximum Likelihood Training for Text Generation with Density Ratio Estimation

Auto-regressive sequence generative models trained by Maximum Likelihood Estimation suffer the exposure bias problem in practical finite sample scenarios. The crux is that the number of training samples for Maximum Likelihood Estimation is usually limited and the input data distributions are different at training and inference stages. Many method shave been proposed to solve the above problem (Yu et al., 2017; Lu et al., 2018), which relies on sampling from the non-stationary model distribution and suffers from high variance or biased estimations. In this paper, we propose{\psi}-MLE, a new training scheme for auto-regressive sequence generative models, which is effective and stable when operating at large sample space encountered in text generation. We derive our algorithm from a new perspective of self-augmentation and introduce bias correction with density ratio estimation. Extensive experimental results on synthetic data and real-world text generation tasks demonstrate that our method stably outperforms Maximum Likelihood Estimation and other state-of-the-art sequence generative models in terms of both quality and diversity.

==> augmented.tex <==
\subsection{Augmented objective for Sequence Generative Modeling}
\label{augmented_obj}
% \citep{grover2019bias} shows that the generative model can be combined in a boosting-like fashion to improve the overall performance. 

% introduced the approach for creating an ensemble of generative models by unsupervised boosting. Inspired by the intuition

In this section, we introduce \emph{additive boosting} for the problem of sequence generative modeling and show that many existing methods can be derived within this framework. 


Note that the goal of sequence generation task is to learn  a conditional probability distribution of the ($l+1$)-th element $S_{l+1}$ in the sentence given the prefix (what has been generated so far) $S_{1:l} = (S_1, \cdots, S_l)$. Here the upper case $S$ is utilized to denote the corresponding discrete random variable in the dataset \lantao{a RV is not in the dataset, it is a RV that can take values in some vocabulary with some distribution}\yuxuan{i see}. With a training data-set $D$ with sentences of length $L$, the standard objective for sequence generation can be further illustrated as follows:
\begin{equation}
\label{teacher forcing}
L_{\mathrm{MLE}}=\underset{S_{1 : L} \sim D}{\mathbb{E}}-\frac{1}{L} \sum_{l=1}^{L} \log G_{\theta}\left(S_{l} | S_{1 : l-1}\right)
\end{equation}\lantao{$L_{\mathrm{MLE}} \to L_{\mathrm{MLE}}(\theta)$}
% Note that in analysis we assume all sentences are of length $L$ for simplicity.
The forced exposure to the ground-truth data as Eq.~\ref{teacher forcing} is known as "teach forcing". Due to the limited training samples, the model are only guaranteed to perform well on the finite samples and during the test or generation time the error may accumulate along the sequence results in a distorted generated distribution. The error accumulation effect origins from both the property of autoregressive model and the poor generalization guarantee within the  limited samples scenario. A crucial property of a generative model is the samples can be easily acquired from the sampling procedure. Note that an important application of generative model is that in supervised learning scenario, samples from a well learned generative model can be augmented into the training set to improve the generalization ability\citep{antoniou2017data}. Hence, there is a strong motivation to explore whether the generated samples can be utilized to improve the training of generative model itself.

A natural attempt is to follow the data augmentation idea, directly mixing the generative distribution and the true data distribution to construct a progressive target:
\begin{equation}
p_{\operatorname{mix}}(S)=m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)
\end{equation}
Where $m \in \left[0,1\right]$ denote the mixture weight. Then at each step, we make the $p_{\operatorname{mix}}$ as the fixed corresponding target, and then minimize the distance or divergence between $p_{\operatorname{mix}}$ and $p_\theta$. Then we will mainly discuss two cases which corresponds to minimizing the reverse Kullback-Leibler(KL) divergence and the forward Kullback–Leibler(KL) divergence and show that many existing works can be generalized into the similar framework.

1) If we seek to minimize the reverse KL divergence between $p_{\operatorname{mix}}$ and $p_\theta$:
\begin{align}
\label{reverse_kl}
L_{G}(\theta)&=\KL\left( p_{\theta}(S)\|p_{\operatorname{mix}}(S)\right) \\ \nonumber
&= \KL\left( p_{\theta}(S)\|m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)\right)
\end{align}
The corresponding objective is equivalent to minimize Skew divergence\citep{lee2001effectiveness} between the $p_{\theta}(S)$ and $p_{\operatorname{data}}(S)$. Recall the definition of Skew divergence:
\begin{equation}
s_{\alpha}(q, r)=\KL(r \| \alpha q+(1-\alpha) r)
\end{equation}
The Skew divergence can be seen as an approximated smooth version of KL divergence, and the weight $\alpha$ controls the degree to which the function approximates $\KL(r \| q)$.  The objective in Eq.~\ref{reverse_kl} can be then written into the form $s_{m}(p_{\mathrm{data}}, p_\theta)$.
Considering the following specific case, \emph{i.e.}, when the mixture weight $m = 1/2$, the objective of Eq.~\ref{reverse_kl} turns into $\KL(p_{\theta}(S)\| 1/2( p_{\mathrm{data}}(S)+ p_{\theta}(S)))$, the objective is essentially minimizing the Jensen Shannon divergence between the generated distribution $p_{\theta}(S)$ and the target distribution $p_{\mathrm{data}}(S)$\citep{goodfellow2014generative,lu2018cot}. 
While optimizing the corresponding target in Eq.~\ref{reverse_kl} can be challenging and many previous works has proposed to address the difficulties.
The key obstacles in the optimization procedure of $L_{G}(\theta)$ lies in the density function of $m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)$ is not available and approximation is needed. There is mainly the following two ways:
\begin{itemize} 
\item The density function of generative model, $G_\theta$ is actually available. To tractably optimize $\KL(p_{\theta}(S)\|m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S))$, COT\citep{lu2018cot} introduce another tractable density model named mediator which is trained to approximate the density $m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)$. And in \citep{li2019adversarial}, the authors substitute the intractable density $p_{\mathrm{data}}$ with  the density of the empirical distribution. 
% In CoT\citep{lu2018cot}, the mixture density is directly estimated with a tractable density mediator $M$. 
\item Instead of directly approximating the density of $m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)$，the density ratio estimation methods can be alternatively applied to estimate the $p_{\theta}(S) /(m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S))$\citep{yu2017seqgan,guo2018long}. 
% \item three \dots{}
\end{itemize}
However, it should be noticed that taking  the gradient of $L_{G}(\theta)$ in Eq.~\ref{reverse_kl} is not trivial as the it incorporated expectation over the learned distribution $p_\theta$. We expand the derivation at here:
\begin{align}
% \end{align}
&\nabla_\theta \KL\left( p_{\theta}(S)\|m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)\right) \nonumber \\ 
&= \nabla_\theta  \underset{S \sim p_{\theta}}{\mathbb{E}}\left[\log \frac{p_{\theta}\left(S\right)}{m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)}\right]
\end{align}
For the simplicity of notations, let:
\begin{equation}
J_\theta\left(S\right)=\log \frac{p_{\theta}\left(S\right)}{m p_{\mathrm{data}}(S)+(1-m) p_{\theta}(S)}
\end{equation}
Then:
\begin{align}
    &\nabla_\theta  \underset{S \sim p_{\theta}}{\mathbb{E}}\left[J_\theta\left(S\right)\right]\nonumber \\
    &=\sum_{S}\left(\nabla_{\theta} p_{\theta}\left(S\right) J_\theta\left(S\right)+p_{\theta}\left(S\right) \nabla_{\theta} J_\theta\left(S\right)\right)\nonumber \\
    &= \sum_{S}p_\theta(S)\left(\nabla_{\theta} \log p_{\theta}\left(S\right) J_\theta\left(S\right)+ \nabla_{\theta} J_\theta\left(S\right)\right) \nonumber \\
    &=  \underset{S \sim p_{\theta}}{\mathbb{E}}\left(\nabla_{\theta} \log p_{\theta}\left(S\right) J_\theta\left(S\right)+ \nabla_{\theta} J_\theta\left(S\right)\right)
\end{align}
The last equation is also known as the score function estimator or REINFORCE\citep{sutton2000policy}.
All the above mentioned works based on the above forward KL optimization will need to back-propagate the gradients estimated by REINFORCE or directly deal with the $\nabla_{\theta} p_{\theta}\left(S\right)$ term by continuous relaxation. Due to the property of high-dimensional discrete data, both two approximation methods will result in highly sub-optimal solution, \emph{i.e.}, can not actually outperform MLE\citep{caccia2018language}. 

2) Optimizing the forward KL divergence between $p_{\operatorname{mix}}(S)$ and $p_\theta(S)$ does not catches much attention.  It has the appealing property of being easily optimized, \emph{e.g.}, the samples from $p_{\operatorname{mix}}(S)$ can be easily acquired through two-step sampling and the optimization does not need the density of $p_{\operatorname{mix}}(S)$.


In  next section, we first show that the above mentioned self-augmentation objectives has strong connections with additive boosting algorithms. And inspired by boosting and density ratio estimation, we propose a method by constructing a "debiased" progressive target for improving neural sequence generation. 

\section{Progressive Bias Correction for Sequence Generation}
Though the additive boosting target $p_{\mathrm{mix}}$ provides the direction of improvement, as introduced above, there may result in slow optimization procedure due to the gap between $p_\theta$ and $p_{\mathrm{data}}$. We formalized the underlying reason of above phenomenon as there exhibits \emph{bias} in the optimization target Eq.~\ref{mle}.
We  claim that there exists \emph{bias} in a expectations-based target when the distribution $p$ under which we actually seek expectations differs from the target distribution $p_{\mathrm{target}}$. In the above mentioned task, we want to conduct MLE under the real data distribution, $\hat{p_{\mathrm{data}}}$, instead we actually conduct MLE under an additive mixture $p_{\mathrm{mix}}$ of the empirical data distribution $p_{\mathrm{data}}$ and the intermediate generated distribution $p_\theta$.

Then a natural question to ask is that given samples from $p_{\mathrm{mix}}$ available, can we use these samples to provide a less biased optimization target further a better gradient direction for updating parameters of generator? 
Inspired by the recent advancements in bias correction for learned generative model\citep{grover2019bias} and likelihood-ratio policy gradient ratio\citep{jie2010connection}, we introduced a bias corrected progressive target for training sequence generation model.  

We are interested in estimate and optimize expectations of a class of functions of interest $f \in \mathcal{F}$ w.r.t to some distribution $p$:
\begin{equation}
\mathrm{E}_{p(X)}[f(X)]=\int_{x} p(x) f(x) d x
\end{equation}
Note that MLE objective corresponds to the situation when $p \equiv p_{\text {data }}$, $f(x) \equiv \log(p_\theta(x))$.  If finite samples from $p$ is available, we can use the sample average of the finite samples as the evaluation results or the optimization target. In the sequence generation scenario mentioned above, we expect to utilize a mixed distribution $p_{\operatorname{mix}}$ to improve the optimization procures towards an expectation of $p_{\text{data}}$. When the discrepancy between $p_{\operatorname{mix}}$ and $p_{\text {data }}$ can not be ignored, an unbiased estimation of $p_{\text{data}}$ with samples from $p_{\operatorname{mix}}$ can be implementation within an importance sampling fashion:
\begin{equation}
\begin{aligned}
&\mathrm {E}_{p_{\text {data }}(S)}[\log p_\theta(S)]=\mathrm{E}_{p_{\operatorname{mix}}(S)}[\frac{p_{\text {data }}(S)}{p_{\operatorname{mix}}(S)}\log p_\theta(S)] \\
& \approx \frac{1}{T} \sum_{i=1}^{T} \frac{p_{\text {data }}\left(s^{(i)}\right)}{p_{\operatorname{mix}}\left(s^{(i)}\right)} \log p_\theta\left(s^{(i)}\right) \text { with } s^{(i)} \sim p_{\operatorname{mix}}(S)
\end{aligned}
\end{equation}

Here the condition that the support of $p_{\text {data }}$ is covered by the support of $p_{\operatorname{mix}}$, \emph{i.e.} $p_{\operatorname{mix}}(S) = 0 \rightarrow p_{\text {data }}(S)$, is satisfied according to the definition of $p_{\operatorname{mix}}$. Therefore, we can first sample from $p_{\operatorname{mix}}$ by  ancestral sampling from $p_\theta$, uniform sampling in the empirical distribution $p_{\text{data}}$ and mixing the samples according to the mixture weight $m$. And then we simply re-weight the samples to obtain an unbiased estimate.

